Extreme Compression for Pre-trained Transformers Made Simple and Efficient

Extreme compression, particularly ultra-low bit precision (binary/ternary) quantization, has been proposed to fit large NLP models on resource-constraint devices. However, to preserve the accuracy for such aggressive compression schemes, cutting-edge methods usually introduce complicated compression pipelines, e.g., multi-stage expensive knowledge distillation with extensive hyperparameter tuning. Also, they oftentimes focus less on smaller transformer models that have already been heavily compressed via knowledge distillation and lack a systematic study to show the effectiveness of their methods. In this paper, we perform a very comprehensive systematic study to measure the impact of many key hyperparameters and training strategies from previous works. As a result, we find out that previous baselines for ultra-low bit precision quantization are significantly under-trained. Based on our study, we propose a simple yet effective compression pipeline for extreme compression, named XTC. XTC demonstrates that (1) we can skip the pre-training knowledge distillation to obtain a 5-layer BERT while achieving better performance than previous state-of-the-art methods, e.g., the 6-layer TinyBERT; (2) extreme quantization plus layer reduction is able to reduce the model size by 50x, resulting in new state-of-the-art results on GLUE tasks.

==> tables/1-bit-bert-base-lr2.tex <==
\begin{table}[ht]
\caption{\textbf{1-bit} quantization for BERT$_{\text{base}}$ with three different KD methods.  }
\centering
\label{table:1-bit-bert-lr1}
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{lcccccccccccccccc }
\toprule
\# & Stages    & learning    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. &Avg. w/o      \\
 &       &     rate &  Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc & Pear/Spea  &      &  CoLA   \\ 
\midrule
 1          & \multirow{4}{*}{One-Stage}  &  2e-5  & 57.3  & 84.1/84.0  & 90.7/86.5  & 91.0  & 88.2/91.2  & 74.0  & 93.1  & 89.2/88.8  & 83.38 & 86.64 \\ 
 2                       &                & 1e-4   & 55.6  & 84.2/84.4  & 90.4/86.0  & 90.4  & 88.3/91.3  & 73.6  & 93.0  & 88.8/88.4  & 83.03 & 86.46 \\ 
  3                      &                & 5e-4   & 46.1  & 82.8/82.9  & 89.9/86.0  & 89.5  & 87.7/90.8  & 71.1  & 92.4  & 88.2/88.0  & 81.09 & 85.46 \\ \cdashline{3-13}
 4                    &           &  Best (above)  & 57.3  & 84.2/84.4  & 90.7/86.5  & 91.0  & 88.3/91.3  & 74.0  & 93.1  & 89.2/88.8  & 83.44 & 86.71 \\ \cline{2-13}
%==============================================================
% NeurIPS_May6_BertBase_2e-05_none_budgetC two_stage 1
 5         & \multirow{4}{*}{Two-Stage}  &  2e-5  & 55.9  & 84.2/83.9  & 90.6/86.5  & 90.7  & 88.3/91.3  & 73.3  & 93.1  & 89.2/88.9  & 83.12 & 86.52 \\ 
6                        &                & 1e-4   & 52.0  & 83.2/83.8  & 90.9/86.5  & 90.1  & 88.0/91.0  & 74.0  & 93.1  & 87.8/87.8  & 82.39 & 86.19 \\ 
7                        &                & 5e-4   & 32.2  & 79.3/80.3  & 90.6/86.5  & 89.6  & 85.3/89.1  & 70.0  & 91.2  & 87.0/86.8  & 78.36 & 84.12 \\ \cdashline{3-13}
8                     &           &  Best (above)  & 55.9  & 84.2/83.9  & 90.6/86.5  & 90.7  & 88.3/91.3  & 74.0  & 93.1  & 89.2/88.9  & 83.20 & 86.61 \\ \cline{2-13}
%==============================================================
% NeurIPS_May6_BertBase_2e-05_none_budgetC three_stage 1
9          & \multirow{4}{*}{Three-Stage}  &  2e-5  & 57.1  & 84.0/84.4  & 90.6/86.5  & 90.9  & 88.1/91.1  & 72.6  & 92.9  & 89.5/89.2  & 83.22 & 86.49 \\ 
10                        &                & 1e-4   & 53.8  & 83.5/84.1  & 90.8/86.8  & 90.1  & 88.3/91.3  & 72.6  & 92.8  & 88.2/87.9  & 82.58 & 86.18 \\ 
11                        &                & 5e-4   & 31.3  & 80.0/81.3  & 89.8/85.3  & 89.2  & 86.7/90.0  & 70.8  & 91.3  & 86.4/86.8  & 78.40 & 84.29 \\ \cdashline{3-13}
 12                    &           &  Best (above)  & 57.1  & 84.0/84.4  & 90.8/86.8  & 90.9  & 88.3/91.3  & 72.6  & 92.9  & 89.5/89.2  & 83.28 & 86.55 \\ 
%==============================================================
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/1-bit-bert-base.tex <==
%%  num_param: 85526016
%%  lora_prarm 8: 1339392;
%%  lora_prarm 4: 669696;
%%  lora_prarm 2: 334848;
%%  lora_prarm 1: 167424;
% \begin{table}[ht]
% \caption{1-bit quantization for BERT$_{\text{base}}$ with size $13.0$MB ($\times 32.0$ smaller than the fp32 version).}
% \centering
% \label{tab:bert_main_result}
% \begin{adjustbox}{width=0.99\linewidth}
% \centering
% \begin{tabular}{llcccccccccccccc }
% \toprule
% \# & Cost    & Stages    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. &Avg.     \\
% & Quantization        &      &  Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &      &  CoLA   \\ 
% \cdashline{1-13}
% % \multicolumn{13}{c}{Training Budget A}\\
% % 3 & TernaryBERT~\cite{zhang-etal-2020-ternarybert} &26.1 ($\times 16.0$)& 55.7  & 83.3/83.3  & 91.2/87.5  & 91.1  & 86.7/90.1  & 72.9  & 93.5  & 92.8/87.9  & 82.70 & 86.11\\\cdashline{1-13} 
% % NeurIPS_May5_BertBase_2e-05_none_budgetA one_stage
%  2 & \multirow{3}{*}{Budget-A}&  One-Stage   & 44.6  & 83.1/83.7  & 88.8/83.1  & 90.5  & 87.4/90.7  & 66.1  & 92.8  & 87.8/87.5  & 80.27 & 84.72 \\ 
% % NeurIPS_May5_BertBase_2e-05_none_budgetA two_stage
% 2 &                          &  Two-Stage    & 48.2  & 83.3/83.8  & 89.3/84.6  & 90.7  & 87.7/90.9  & 70.4  & 92.5  & 88.7/88.4  & 81.46 & 85.61 \\ 
% % NeurIPS_May5_BertBase_2e-05_none_budgetA three_stage
% 2 &                         &  Three-Stage   & 49.3  & 83.1/83.6  & 89.5/84.3  & 90.9  & 87.6/90.9  & 70.8  & 92.4  & 88.7/88.3  & 81.56 & 85.59 \\ \cdashline{1-13} 
% % NeurIPS_May5_BertBase_2e-05_none_budgetB one_stage
% 6 &  \multirow{3}{*}{Budget-B} & One-Stage   & 51.8  & 84.1/84.4  & 89.6/84.6  & 90.4  & 88.0/91.1  & 70.8  & 92.8  & 88.8/88.4  & 82.09 & 85.88 \\ 
% % NeurIPS_May5_BertBase_2e-05_none_budgetB two_stage
% 6 &                             & Two-Stage  & 52.4  & 84.0/84.5  & 89.7/85.0  & 90.2  & 88.0/91.1  & 72.2  & 92.7  & 89.2/88.8  & 82.37 & 86.11 \\ 
% % NeurIPS_May5_BertBase_2e-05_none_budgetB three_stage
% 6 &                             &Three-Stage & 53.0  & 83.8/84.4  & 90.1/85.3  & 90.7  & 88.0/91.1  & 72.2  & 93.2  & 89.2/88.8  & 82.54 & 86.24 \\ \cdashline{1-13} 
% 6 &\multirow{3}{*}{Budget-C}   &    One-Stage & 57.3  & 84.0/84.4  & 90.8/86.5  & 90.6  & 88.2/91.2  & 74.0 & 93.1  & 89.2/88.8  & \textbf{83.37} & \textbf{86.62}\\
% 6 &                            &    Two-Stage & 57.0  & 84.2/84.3  & 90.6/86.5  & 90.8  & 88.0/91.1  & 73.3  & 93.0  & 89.0/88.7  & 83.24 & 86.53 \\
% 6 & & Three-Stage        & \textbf{57.5} & 84.1/84.3  & \textbf{91.1/87.0} & 90.8  & 88.2/91.2  & 72.9& 93.2 & 89.1/88.8  & 83.34 & 86.58 \\ % 
% % 5 & 1-bit (One-Stage         & \multirow{3}{*}{13.0 ($\times 32.0$)}   & 53.8  & 84.1/84.0  & 90.1/85.5  & 91.0  & 88.2/91.2  & 73.3  & 92.7  & 89.1/88.8  & 82.74 & 86.36 \\ 
% % 6 & 1-bit (Two-Stage         &                                         & 55.2  & 84.2/84.3  & 90.3/86.0  & 90.7  & 88.0/91.1  & 72.2  & 92.9  & 89.4/89.0  & 82.89 & 86.35 \\
% % 6 & 1-bit (Three-Stage         &                                         & 55.1  & 84.1/84.6  & 89.9/85.3  & 91.1  & 88.1/91.2  & 73.3  & 92.9  & 89.2/88.9  & 82.98 & 86.46 \\\cdashline{1-13}
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}
\begin{table}[ht]
\caption{\textbf{1-bit or 2-bit} quantization for \bertbase with various Budget-A, Budget-B and Budget-C}%with size $13.0$MB ($\times 32.0$ smaller than its fp32 version)
\centering
\label{table:1-bit-bert}
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{llcccccccccccccc }
\toprule
\# & Cost    & Stages    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. & Avg. w/o     \\
&        &  & Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &      &  CoLA   \\ 
\midrule
0 & \multicolumn{2}{c}{BERT$_{\text{base}}$ (fp32) }         &  59.7  &  84.9/85.6   &  90.6/86.3  &  92.1  &  88.6/91.5   & 72.2   & 93.2  & 90.1/89.6 & 83.95 & 86.98\\\midrule
1 &\multirow{2}{*}{Budget-A} 
             &      One-Stage   & 50.4  & 83.7/84.6  & 90.0/85.8  & 91.3  & 88.0/91.1  & 72.9  & 92.8  & 88.8/88.4  & 82.38 & 86.37 \\ 
%==============================================================
2 &  \multirow{2}{*}{(1-bit)}           &      Two-Stage   & 48.5  & 83.3/83.8  & 90.0/85.5  & 90.7  & 87.7/90.9  & 70.4  & 92.5  & 88.7/88.4  & 81.59 & 85.72 \\ 
%==============================================================
3 &          &      Three-Stage   & 49.3  & 83.2/83.4  & 89.7/84.8  & 91.0  & 87.6/90.9  & 73.6  & 92.4  & 88.8/88.5  & 81.93 & 86.01 \\ 
%==============================================================
\cdashline{1-13}
4 &\multirow{2}{*}{Budget-B} 
             &      One-Stage   & 55.6  & 84.1/84.4  & 90.4/86.0  & 90.8  & 88.3/91.3  & 72.6  & 93.1  & 88.9/88.5  & 82.98 & 86.40 \\ 
%==============================================================
5 &  \multirow{2}{*}{(1-bit)}          &      Two-Stage   & 52.4  & 84.0/84.5  & 90.3/85.8  & 90.5  & 88.0/91.1  & 72.9  & 92.7  & 89.2/88.8  & 82.57 & 86.34 \\ 
%==============================================================
6 &          &      Three-Stage   & 53.0  & 83.8/84.4  & 90.4/86.0  & 90.7  & 88.0/91.1  & 72.6  & 93.2  & 89.2/88.8  & 82.67 & 86.38 \\ 
%==============================================================
\cdashline{1-13}
7 &\multirow{2}{*}{Budget-C} 
             &      One-Stage   & 57.3  & 84.2/84.4  & 90.7/86.5  & 91.0  & 88.3/91.3  & 74.0  & 93.1  & 89.2/88.8  & 83.44 & 86.71 \\ 
%==============================================================
8 &  \multirow{2}{*}{(1-bit)}         &      Two-Stage   & 55.9  & 84.2/83.9  & 90.6/86.5  & 90.7  & 88.3/91.3  & 74.0  & 93.1  & 89.2/88.9  & 83.20 & 86.61 \\ 
%==============================================================
9 &          &      Three-Stage   & 57.1  & 84.0/84.4  & 90.8/86.8  & 90.9  & 88.3/91.3  & 72.6  & 92.9  & 89.5/89.2  & 83.28 & 86.55 \\ 
%==============================================================
\midrule

10 &\multirow{2}{*}{Budget-A} 
             &      One-Stage   & 58.0  & 84.5/85.0  & 90.9/87.0  & 91.5  & 88.4/91.4  & 74.0  & 93.5  & 89.6/89.2  & 83.83 & 87.06 \\ 
%==============================================================
11 & \multirow{2}{*}{(2-bit)}          &      Two-Stage   & 56.6  & 84.3/85.0  & 91.0/87.3  & 91.3  & 88.3/91.3  & 72.2  & 93.5  & 89.6/89.1  & 83.46 & 86.81 \\ 
%==============================================================
12 &          &      Three-Stage   & 58.8  & 84.3/84.7  & 90.4/86.8  & 91.4  & 88.0/91.2  & 74.0  & 93.5  & 89.6/89.1  & 83.81 & 86.94 \\ 
%==============================================================
\cdashline{1-13}
13 &\multirow{2}{*}{Budget-B} 
             &      One-Stage   & 58.2  & 84.6/84.7  & 91.3/87.7  & 91.4  & 88.4/91.4  & 75.8  & 93.5  & 89.6/89.2  & 84.10 & 87.34 \\ 
%==============================================================
14 &  \multirow{2}{*}{(2-bit)}           &      Two-Stage   & 58.4  & 84.3/84.9  & 91.1/87.3  & 91.4  & 88.4/91.3  & 74.0  & 93.5  & 89.7/89.4  & 83.87 & 87.05 \\ 
%==============================================================
15 &          &      Three-Stage   & 59.6  & 84.6/84.8  & 90.9/86.5  & 91.3  & 88.3/91.4  & 74.4  & 93.3  & 89.7/89.3  & 83.96 & 87.00 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/1-bit-bert6.tex <==
\begin{table}[ht]
\caption{Comparisons between TinyBERT with other baselines on the dev set of GLUE tasks. Mcc refers to Matthews correlation and Pear/Spea refer to Pearson/Spearman.}
%%  num_param: 
%%  lora_prarm 8: 1339392;
%%  lora_prarm 4: 669696;
%%  lora_prarm 2: 334848;
%%  lora_prarm 1: 167424;
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{lccccccccccccccc }
\toprule
Model    &  size    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. &Avg. w/o      \\
&  (MB)    & (8.5k) &  (393k)     & (3.7k)     & (105k) &  (364k)     & (2.5k) & (67k) &  (5.7k)    & all  & without \\ 
    &      &  Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &      &  CoLA   \\   \midrule    
BERT-{base} fp32             & 417.2   &  59.7  &  84.9/85.6   &  90.6/86.3  &  92.1  &  88.6/91.5   & 72.2   & 93.2  & 90.1/89.6 & 83.95 & 86.98\\\midrule
TinyBERT$_{6}$ (\cite{jiao-etal-2020-tinybert}-v3) & 255.2 ($\times 1.6$)   &  54.0  &  84.5/84.5   &  90.6/86.3  &  91.1  &  88.0/91.1   & 70.4   & 93.0  & 90.1/89.6 & 82.78 & 86.38\\
TinyBERT$_{6}$ (reproduce*)  & 255.2 ($\times 1.6$)   &  56.9  &  84.4/84.8   &  90.1/85.5  &  91.3  &  88.4/91.4   & 72.2   & 93.2  & 90.3/90   & 83.33 & 86.64 \\ \cdashline{1-12}
1-bit (1-Stage)  & 8.0 ($\times 52.3$)   & 48.8  & 82.7/82.9  & 89.0/83.8  & 89.4  & 87.8/90.9  & 67.5  & 92.4  & 87.0/86.7  & 80.6 & 84.58 \\  
1-bit (2-Stage)  & 8.0 ($\times 52.3$)   & 48.9  & 82.8/83.1  & 89.9/85.3  & 89.2  & 87.8/90.9  & 66.1  & 93.0  & 87.3/86.9  & 80.73 & 84.71 \\ 
1-bit (3-Stage)  & 8.0 ($\times 52.3$)   & 49.1  & 82.9/83.7  & 88.9/83.8  & 89.4  & 87.9/91.0  & 65.7  & 92.7  & 87.1/86.7  & 80.6 & 84.54 \\   \cdashline{1-12}
SkipBERT$_{6}$ (3-stage)                & 255.2 ($\times 1.6$) & 56.1  & 84.4/84.5  & 90.5/86.0  & 91.6  & 88.3/91.4  & 73.6  & 93.5  & 89.3/88.9  & 83.38 & 86.79 \\ 
1-bit+LoRA8 (3-Stage) &  9.3 ($\times 45.0$) & 52.2  & 82.9/83.3  & 90.2/85.8  & 89.7  & 87.8/90.9  & 67.5  & 92.8  & 88.4/88.1  & 81.5 & 85.16 \\ \cdashline{1-12}
1-bit (1-Stage)  & 8.0 ($\times 52.3$) & 51.5  & 83.0/83.1  & 89.8/84.8  & 89.2  & 87.9/91.0  & 66.4  & 92.9  & 88.2/87.8  & 81.12 & 84.83 \\ 
1-bit (2-Stage)  & 8.0 ($\times 52.3$) & 51.6  & 82.7/83.6  & 89.7/84.8  & 88.8  & 87.9/91.0  & 66.4  & 92.9  & 88.2/87.8  & 81.11 & 84.8 \\
1-bit (3-Stage) &  8.0 ($\times 52.3$) & 51.1  & 82.7/83.5  & 89.9/85.0  & 89.4  & 88.0/91.0  & 67.5  & 92.8  & 88.0/87.7  & 81.28 & 85.05 \\ % \cdashline{1-12}
% 1-bit+(a)+(b4) & 8.6 ($\times 48.4$)  &  \\  
% 1-bit+(a)+(b2) & 8.3 ($\times 50.3$)  & \\
  \midrule
1-bit (1-Stage)(longer) &  8.0 ($\times 52.3$) & 52.7  & 82.9/83.7  & 90.9/86.8  & 89.5  & 87.9/91.0  & 67.5  & 92.9  & 88.4/88.1  & 81.71 & 85.34 \\ 
1-bit (2-Stage)(longer) &  8.0 ($\times 52.3$)  & 53.2  & 82.7/83.1  & 90.7/86.5  & 88.9  & 87.9/91.0  & 68.2  & 92.9  & 88.2/87.9  & 81.63 & 85.19 \\ 
1-bit (3-Stage)(longer) &  8.0 ($\times 52.3$) & 53.8  & 83.0/83.4  & 90.9/86.8  & 89.0  & 88.0/91.1  & 66.4  & 93.1  & 88.4/88.0  & 81.67 & 85.15 \\ 
 \cdashline{1-12} % not finished  qnli, mnli, qqp, sst-2
  1-bit+(b1) (1-Stage)(longer)    & 8.1 ($\times 51.3$) & 53.6  & 83.4/83.8  & 90.7/86.5  & 89.5  & 87.5/90.7  & 67.9  & 93.0  & 88.4/88.0  & 81.87 & 85.40 \\
1-bit+(b1) (2-Stage)(longer)    & 8.1 ($\times 51.3$)& 53.3  & 82.8/83.3  & 91.2/87.3  & 89.0  & 87.9/91.0  & 67.5  & 92.8  & 88.2/87.8  & 81.69 & 85.24 \\ 
 1-bit+(b1) (3-Stage)(longer)    & 8.0 ($\times 52.3$)  & 53.2  & 83.5/83.7  & 90.8/86.5  & 89.1  & 88.0/91.1  & 66.8  & 92.8  & 88.3/88.0  & 81.67 & 85.22 \\   \midrule
 1-bit (3-stage*) & 8.0 ($\times 52.3$) & 53.8  & 82.8/83.6  & 91.2/87.3  & 89.4  & 88.0/91.1  & 67.5  & 92.9  & 88.1/87.7  & 81.83 & 85.34 \\  % not yet finished
Continue a second 3-Stage*\\
1-bit+(vanilla) & 8.0 ($\times 52.3$) & 53.8  & 83.1/83.7  & 90.6/86.3  & 89.3  & 88.0/91.1  & 68.6  & 93.0  & 88.2/87.9  & 81.90 & 85.41 \\   
1-bit+(b1) & 8.1 ($\times 51.3$)  & 53.9  & 83.4/83.8  & 90.9/86.8  & 90.0  & 88.1/91.2  & 68.6  & 93.1  & 88.3/87.9  & \textbf{82.12} & \textbf{85.65} \\
% 1-bit+(a)      & 8.0 ($\times 52.3$) & \\
1-bit+(b8)     & 9.3 ($\times 45.0$) & 53.8  & 83.1/83.8  & 90.9/86.8  & 90.0  & 88.1/91.1  & 68.2  & 92.9  & 88.3/87.9  & 82.00 & 85.52 \\ 
1-bit+(a)+(b8) & 9.3 ($\times 45.0$) & 53.7  & 83.0/83.9  & 91.1/87.3  & 89.1  & 88.0/91.1  & 67.9  & 92.9  & 88.3/88.0  & 81.91 & 85.44 \\ 
 \multicolumn{8}{l}{The above are all based on a \textbf{3-stage} fp16 checkpoint}\\
 \midrule
 \multicolumn{8}{l}{The following are based on a \textbf{1-stage} fp16 checkpoint}\\
  SkipBERT$_{6}$ (1-stage long)                 & 255.2 ($\times 1.6$) &  57.0  & 84.4/84.6  & 90.5/86.0  & 91.5  & 88.4/91.5  & 72.6  & 93.5  & 89.3/88.9  & 83.38 & 86.67 \\ 
 2-bit (1-Stage)(short)      & 16.0 ($\times 26.2$)  &  54.1  & 83.8/83.6  & 90.5/86.3  & 90.9  & 88.2/91.3  & 70.4  & 93.3  & 88.8/88.5  & 82.50 & 86.05 \\
 2-bit+(b8) (1-Stage)(short) & 18.6 ($\times 22.5$) & 54.0  & 83.6/84.3  & 91.0/86.8  & 91.0  & 88.3/91.3  & 70.4  & 93.3  & 88.9/88.5  & 82.62 & 86.20  \\  \cdashline{1-12}
1-bit (1-Stage)(short)      & 8.0 ($\times 52.3$)  &  51.1  & 83.2/83.5  & 89.3/84.3  & 89.3  & 87.9/91.0  & 65.0  & 92.9  & 88.2/87.8  & 80.94 & 84.68 \\ 
1-bit+ (b1)(1-Stage)(short) & 8.1 ($\times 51.3$) & 51.6  & 83.1/83.6  & 89.6/84.8  & 89.5  & 87.9/91.0  & 64.3  & 92.7  & 88.3/87.9  & 80.99 & 84.66 \\ 
1-bit+ (b8)(1-Stage)(short) & 9.3 ($\times 45.0$) &  51.1  & 83.2/83.7  & 89.9/85.0  & 89.8  & 87.7/90.9  & 64.6  & 92.9  & 88.3/88.0  & 81.06 & 84.80 \\ 
% NeurIPS_April29myBERTskipCORRECT_BertBase_newStage_longer one_stage
1-bit (1-Stage)(long)       & 8.0 ($\times 52.3$)   &  52.3  & 83.3/83.6  & 90.4/86.0  & 89.1  & 87.9/91.0  & 66.8  & 93.0  & 88.6/88.2  & 81.52 & 85.17 \\ 
1-bit+ (b1)(1-Stage)(long)  & 8.1( $\times 51.3$) & 53.7  & 83.1/83.3  & 90.6/86.3  & 89.7  & 87.8/91.0  & 67.5  & 93.0  & 88.5/88.1  & 81.79 & 85.30 \\ 
1-bit+ (b8)(1-Stage)(long)  & 9.3 ($\times 45.0$)& 52.7  & 83.3/83.6  & 90.1/85.3  & 89.5  & 87.9/91.0  & 67.1  & 92.9  & 88.6/88.3  & 81.56 & 85.16 \\  \bottomrule
%  1-bit (3-Stage)(ours) &  8.0 ($\times 52.3$)   & 53.8  & 82.8/83.6  & 91.2/87.3  & 88.8  & 88.0/91.1  & 67.5  & 92.9  & 88.1/87.7  & 81.77 & 85.26 \\ 
%  				SkipBERT$_{6}$+loRA              &  {55.95}  &  {84.49/84.51}   & {90.33/85.78} &  {91.62}  & {88.46/91.51} & {72.92}   & {93.58}  & {89.25/88.9} &83.29& 86.71
%  \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/2-bit-bert-base.tex <==
%%  num_param: 85526016
%%  lora_prarm 8: 1339392;
%%  lora_prarm 4: 669696;
%%  lora_prarm 2: 334848;
%%  lora_prarm 1: 167424;
% \begin{table}[ht]
% \caption{Ternary Quantization for BERT$_{\text{base}}$
% }
% \centering
% \label{tab:bert_main_result}
% \begin{adjustbox}{width=0.99\linewidth}
% \centering
% \begin{tabular}{llcccccccccccccc }
% \toprule
% Cost    & \# &  Stages    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. &Avg.     \\
% &       &      &  Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &      &  CoLA   \\ 
% \midrule
% % \multicolumn{13}{c}{Training Budget A}\\
% % 3 & TernaryBERT~\cite{zhang-etal-2020-ternarybert} &26.1 ($\times 16.0$)& 55.7  & 83.3/83.3  & 91.2/87.5  & 91.1  & 86.7/90.1  & 72.9  & 93.5  & 92.8/87.9  & 82.70 & 86.11\\\cdashline{1-13} 
% 2 & \multirow{3}{*}{Budget-A}&  One-Stage & 58.0  & 84.2/84.6  & 89.8/84.8  & 91.5  & 88.4/91.4  & 72.2  & 93.5  & 89.4/89.0  & 83.29 & 86.45 \\ 
% 2 & &  Two-Stage         & 56.6  & 84.3/85.0  & 91.0/87.3  & 91.3  & 88.3/91.3  & 71.5  & 93.5  & 89.6/89.1  & 83.38 & 86.73 \\ 
% 2 & &  Three-Stage      & 58.8  & 84.3/84.7  & 90.4/86.8  & 91.4  & 88.0/91.2  & 72.6  & 93.5  & 89.6/89.1  & 83.66 & 86.76 \\\midrule 
% 6 &  \multirow{3}{*}{Budget-B} & One-Stage & 58.2  & 84.6/84.7  & 91.3/87.7  & 91.3  & 88.4/91.4  & 73.6  & 93.3  & 89.6/89.2  & 83.82 & 87.03 \\   
% 6 &                          & Two-Stage  & 58.4  & 84.3/84.9  & 90.5/86.3  & 91.2  & 88.4/91.3  & 74.0  & 93.5  & 89.7/89.4  & 83.73 & 86.90 \\  
% 6 &                          & Three-Stage  & 59.6  & 84.5/84.7  & 90.9/86.5  & 91.3  & 88.3/91.3  & 73.3  & 93.3  & 89.7/89.3  & 83.80 & 86.83 \\    \midrule 


% 6 &\multirow{3}{*}{Budget-C} & One-Stage & 59.9  & 84.7/84.4  & 91.0/86.7  & 91.4  & 88.4/91.4  & 74.0  & 93.5  & 89.6/89.2  & 84.00 & 87.01 \\ 
% 6 &                          & Two-Stage  & 59.9  & 84.9/84.7  & 91.2/87.3  & 91.2  & 88.2/91.3  & 73.3  & 93.5  & 89.7/89.4  & 83.98 & 86.99 \\ 
% 6 &                          & Three-Stage   & 59.6  & 84.7/84.3  & 91.0/87.0  & 91.2  & 88.4/91.3  & 74.4  & 93.7  & 89.6/89.2  & 83.98 & 87.03 \\  % 
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}


\begin{table}[ht]
\caption{Ternary Quantization for BERT$_{\text{base}}$
}
\centering
\label{table:2-bit-bert}
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{llcccccccccccccc }
\toprule
\# & Cost    & Stages    &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. &Avg. w/o     \\
&        &  & Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &      &  CoLA   \\ \midrule
0 & \bertbase (fp32)    &na         &  59.7  &  84.9/85.6   &  90.6/86.3  &  92.1  &  88.6/91.5   & 72.2   & 93.2  & 90.1/89.6 & 83.95 & 86.98\\\midrule
1 &\multirow{3}{*}{Budget-A} 
             &      One-Stage   & 58.0  & 84.5/85.0  & 90.9/87.0  & 91.5  & 88.4/91.4  & 74.0  & 93.5  & 89.6/89.2  & 83.83 & 87.06 \\ 
%==============================================================
2 &          &      Two-Stage   & 56.6  & 84.3/85.0  & 91.0/87.3  & 91.3  & 88.3/91.3  & 72.2  & 93.5  & 89.6/89.1  & 83.46 & 86.81 \\ 
%==============================================================
3 &          &      Three-Stage   & 58.8  & 84.3/84.7  & 90.4/86.8  & 91.4  & 88.0/91.2  & 74.0  & 93.5  & 89.6/89.1  & 83.81 & 86.94 \\ 
%==============================================================
\midrule
4 &\multirow{3}{*}{Budget-B} 
             &      One-Stage   & 58.2  & 84.6/84.7  & 91.3/87.7  & 91.4  & 88.4/91.4  & 75.8  & 93.5  & 89.6/89.2  & 84.10 & 87.34 \\ 
%==============================================================
5 &          &      Two-Stage   & 58.4  & 84.3/84.9  & 91.1/87.3  & 91.4  & 88.4/91.3  & 74.0  & 93.5  & 89.7/89.4  & 83.87 & 87.05 \\ 
%==============================================================
6 &          &      Three-Stage   & 59.6  & 84.6/84.8  & 90.9/86.5  & 91.3  & 88.3/91.4  & 74.4  & 93.3  & 89.7/89.3  & 83.96 & 87.00 \\ 
%==============================================================
% \midrule
% 7 &\multirow{3}{*}{Budget-C*}  & One-Stage & 59.9  & 84.7/84.4  & 91.0/86.7  & 91.4  & 88.4/91.4  & 74.0  & 93.5  & 89.6/89.2  & 84.00 & 87.01 \\ 
% 8 &                         & Two-Stage  & 59.9  & 84.9/84.7  & 91.2/87.3  & 91.2  & 88.2/91.3  & 73.3  & 93.5  & 89.7/89.4  & 83.98 & 86.99 \\ 
% 9 &                          & Three-Stage   & 59.6  & 84.7/84.3  & 91.0/87.0  & 91.2  & 88.4/91.3  & 74.4  & 93.7  & 89.6/89.2  & 83.98 & 87.03 \\  % 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/DA-layer-reduction.tex <==
\begin{table}[ht]
\caption{Compare between with and without data augmentation for a smaller \bertbase (six layers)}\label{table:da-fp}
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{lccccccccccccccc }
\toprule
\# & DS-BERT$_6$  & Data   &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B    & Avg. & DIFF \\
  &  Stages  & Aug. & Mcc     &   Acc/Acc   & F1/Acc     &  Acc   &  F1/Acc     & Acc    &  Acc  & Pear/Spea  &    all  &   \\   \midrule  

1 &  \multirow{2}{*}{One-stage }  & \cmark    & 56.9  & 84.5/84.9  & 89.7/84.8  & 91.7  & 88.5/91.5  & 71.8  & 93.5  & 89.8/89.4  & 83.27 & \multirow{2}{*}{-2.18} \\
2&                               & \xmark      & 52.2  & 84.4/84.6  & 88.4/82.4  & 91.4  & 88.4/91.5  & 63.9  & 92.9  & 86.5/86.3  & 81.09 &  \\ \cdashline{1-13}
3 &  \multirow{2}{*}{Two-stage}  & \cmark     & 56.0  & 84.1/84.2  & 89.7/84.8  & 91.5  & 88.2/91.3  & 71.8  & 93.3  & 89.4/89.1  & 82.93 & \multirow{2}{*}{-2.03}  \\  
4&                               & \xmark     & 50.2  & 84.1/84.2  & 88.7/83.1  & 90.8  & 88.2/91.3  & 64.6  & 92.9  & 86.9/86.7  & 80.90 &  \\  %\cdashline{1-13}
% 5 &  \multirow{2}{*}{Three-stage}  & Yes     \\ 
% 6&                               & no    & 51.2  & 84.4/84.5  & 88.3/82.8  & 91.3  & 88.3/91.4  & 64.6  & 92.9  & 87.5/87.3  & 81.18 & 84.92 \\ 
 \bottomrule
\end{tabular}
\end{adjustbox}

\end{table}
%%  num_param: 
%%  lora_prarm 8: 1339392;
%%  lora_prarm 4: 669696;
%%  lora_prarm 2: 334848;
%%  lora_prarm 1: 167424;

==> tables/budget.tex <==
\begin{table}[ht]
\caption{Ternary Quantization for BERT$_{\text{base}}$
}
\centering
\label{table:2-bit-bert}
\begin{adjustbox}{width=0.99\linewidth}
\centering
\begin{tabular}{lccccccccccc}
\toprule
 Training Cost   &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B      \\\midrule
 Budget-A   &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B      \\
 Budget-B  &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B      \\
Budget-C   &  CoLA  & MNLI-m/-mm  &  MRPC      &  QNLI  &    QQP      & RTE    & SST-2 &   STS-B      \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/stages-table.tex <==
% \begin{table}[ht]
% \caption{}
% \begin{adjustbox}{width=0.99\linewidth}
% \begin{tabular}{l|l|l|l }
% \toprule
%  Iterations &                 \multicolumn{1}{c|}{\onestage} &   \multicolumn{1}{c|}{\twostage}  &   \multicolumn{1}{c}{\threestage}  \\\midrule
%  $0-T_1$  &\multirow{3}{*}{Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}+\mathcal{L}_{\text{logit}}$}  &   \multirow{2}{*}{ Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}$}  &   Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}$ (learns feature maps)\\            
% $T_1-T_2$  & &  \multirow{2}{*}{ Stage-II: $\mathcal{L}_{\text{logit}}$}   & Stage-II: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}+\mathcal{L}_{\text{logit}}$ (transition state)\\
% $T_2-T_3$  & &   &  Stage-III: $\mathcal{L}_{\text{logit}}$ (learns prediction)\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{table:ta2}
% \end{table}


% \begin{table}[ht]
% \caption{}
% \begin{adjustbox}{width=0.99\linewidth}
% \begin{tabular}{lcccc}
% \toprule
%  \multirow{2}{*}{Stages}      &   \multicolumn{4}{c}{Training Time}  \\
%                               &  $T_1$  &   $T_1+T_2/2$  &    $T_1+T_2$  &   $T_1+T_2+T_3$  \\ \midrule
% \onestage & \multicolumn{4}{c}{Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}+\mathcal{L}_{\text{logit}}$ }  \\
% \twostage & \multicolumn{2}{c}{Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}$ }&   \multicolumn{2}{c}{Stage-II: $\mathcal{L}_{\text{logit}}$ } \\
%  \threestage &   Stage-I: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}$ & Stage-II: $\mathcal{L}_{\text{hidden}}+\mathcal{L}_{\text{att}}+\mathcal{L}_{\text{logit}}$ &  Stage-III:$\mathcal{L}_{\text{logit}}$ (learns prediction)\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{table:ta2}
% \end{table}
% \begin{itemize}
%     \item Stage-I: 
%     \item Stage-II:
%     \item Stage-III:
% \end{itemize}

